Designing gradient coils with the shape derivative and the closed B-spline curves

This study proposes a versatile and efficient optimisation method for discrete coils that induce a magnetic field by their steady currents. The prime target is gradient coils for MRI (Magnetic Resonance Imaging). The derivative (gradient) of the $z$-component the magnetic field, which is calculated by the Biot--Savart's law, with respect to the $z$-coordinate in the Cartesian $xyz$ coordinate system is considered as the objective function. Then, the derivative of the objective function with respect to a change of coils in shape is formulated according to the concept of shape optimisation. The resulting shape derivative (as well as the Biot--Savart's law) is smoothly discretised with the closed B-spline curves. In this case, the control points (CPs) of the curves are naturally selected as the design variables. As a consequence, the shape derivative is discretised to the sensitivities of the objective function with respect to the CPs. Those sensitivities are available to solve the present shape-optimisation problem with a certain gradient-based nonlinear-programming solver. The numerical examples exhibit the mathematical reliability, computational efficiency, and engineering applicability of the proposed methodology based on the shape derivative/sensitivities and the closed B-spline curves.

==> Makefile <==
SRC = ms.tex #メインのTeXソース
BIB = reference.bib

TEX = platex

yymmdd = $(shell date +%y%m%d_%H%M)

PDF = ${SRC:.tex=.pdf}

all: ${SRC} ${BIB} 
	${TEX} ${SRC} | grep -v "tex/"
	bibtex ${SRC:.tex=.aux}
	${TEX} ${SRC} | grep -v "tex/"
	dvipdfmx ${SRC:.tex=.dvi}
clean:
	rm -f *.dvi *.log *.aux *.lot *.lof *.toc *.bbl *.blg *.spl *.out core
tar:
	tar cvfz ${SRC:.tex=.tgz} Makefile *.tex *.bib *.sty
ax arxiv:
	tar cvfz ${SRC:.tex=.tar.gz} Makefile *.tex *.bbl \
	figure/*.eps \
	240205/check/*.eps \
	240205/gradcoil/*.eps \
	240205/gradcoil2/*.eps \
	240315/gradcoil5/*.eps \
	240315/gradcoil6/*.eps 
b back backup: tar
	mv ${SRC:.tex=.tgz} backup/${yymmdd}.tgz
	cp -p ${PDF} backup/${yymmdd}.pdf
separate sep:
#	rm -f tmptmptmp*.pdf
#	pdfseparate ${PDF} -f 26 -l 26 title.pdf
#	rm -f tmptmptmp*.pdf
#	pdfseparate ${PDF} -f 1 -l 20 tmptmptmp%d.pdf
#	pdfunite tmptmptmp?.pdf manuscript.pdf
	pdfseparate ${PDF} -f 21 -l 24 tmptmptmp%d.pdf
	pdfunite tmptmptmp??.pdf resp.pdf
	rm -f tmptmptmp*.pdf

